Pix4Point: Image Pretrained Standard Transformers for 3D Point Cloud Understanding

While Transformers have achieved impressive success in natural language processing and computer vision, their performance on 3D point clouds is relatively poor. This is mainly due to the limitation of Transformers: a demanding need for extensive training data. Unfortunately, in the realm of 3D point clouds, the availability of large datasets is a challenge, exacerbating the issue of training Transformers for 3D tasks. In this work, we solve the data issue of point cloud Transformers from two perspectives: (i) introducing more inductive bias to reduce the dependency of Transformers on data, and (ii) relying on cross-modality pretraining. More specifically, we first present Progressive Point Patch Embedding and present a new point cloud Transformer model namely PViT. PViT shares the same backbone as Transformer but is shown to be less hungry for data, enabling Transformer to achieve performance comparable to the state-of-the-art. Second, we formulate a simple yet effective pipeline dubbed "Pix4Point" that allows harnessing Transformers pretrained in the image domain to enhance downstream point cloud understanding. This is achieved through a modality-agnostic Transformer backbone with the help of a tokenizer and decoder specialized in the different domains. Pretrained on a large number of widely available images, significant gains of PViT are observed in the tasks of 3D point cloud classification, part segmentation, and semantic segmentation on ScanObjectNN, ShapeNetPart, and S3DIS, respectively. Our code and models are available at https://github.com/guochengqian/Pix4Point .

==> figures/sectionsCVPR/methodology.tex <==
% %------------------------
\input{figures/tex/pipeline}
% %------------------------------------------------------------------------
\section{Methodology}
This section first introduces a new ST-based network called \textit{PViT} that improves the performance of ST for point cloud understanding. 
Then, we present \textit{Pix4Point}, a practical framework that utilizes plentiful available image data to help point cloud tasks. The architecture of PViT and the full pipeline of Pix4Point are illustrated in \figlabel{\ref{fig:pipeline}}.


\subsection{PViT Network}
\label{sec:network}
Inspired by ViT \cite{dosovitskiy2021vit}, Yu \etal designed the first ST-based point cloud network in their PointBERT work  \cite{yu2022pointbert}, which we refer to as vanilla ST throughout texts.
Vanilla ST presents a simple point tokenizer that groups the input point cloud into local patches by a single farthest point sampling (FPS) operation to sample center points, a k-nearest neighbor (kNN) layer to group neighbors, and a mini-PointNet \cite{qi2017pointnet} to project local patches to point tokens. 
This simple extension of ViT \cite{dosovitskiy2021vit} to point clouds achieves rather poor performance in several 3D benchmarks. 
A follow-up work named Point-MAE uses the same vanilla ST model as Point-BERT, but relies on a better SSL method to improve the performance. 
In this work, we propose a new ST model for point clouds called Point Vision Transformer (PViT) that can achieve comparable performance to the state-of-the-art. PViT consists of three modules: a \textit{tokenizer}, an \textit{ST backbone}, and a \textit{task decoder}. 
While the backbone architecture is kept as an unchanged Standard Transformer, the tokenizer and the decoder are specialized to the domain and task. We describe our improved tokenizer and decoder in PViT next.

\minorsection{Tokenizer $\mathbf{t}$: Progressive Point Patch Embedding}
Consider input point cloud $\mathcal{X} \in \mathbb{R}^{N \times (3+C_{in})}$ representing $N$ points with $C_{in}$ input features (\eg colors, normals), the tokenizer $\mathbf{t}$ projects the input point cloud into a sub-cloud (a smaller number of points but in a higher dimensional space). Our \textit{Progressive Point Patch Embedding} (\textit{P3E}) progressively tokenizes point clouds through multiple stages with $\mathbf{t}$: $\mathbb{R}^{N \times (3+C_{in})} \rightarrow \mathbb{R}^{\frac{N}{4} \times \frac{C}{2}} \rightarrow \mathbb{R}^{\frac{N}{16} \times C}$. At each stage, P3E uses FPS to sample a subset of points with a fixed sample ratio ($1/4$), queries neighbors for each downsampled point, and leverages graph convolutions to abstract features to sub-clouds. P3E consists of two FPS stages rather than one in Point-BERT \cite{yu2022pointbert} and Point-MAE \cite{pang2022pointmae}, which is shown to ease the optimization and offers large performance gains in various experiments. The graph convolution in each stage of P3E is defined as Eq. \ref{eqn:tokenizer}:
\begin{equation}\label{eqn:tokenizer}
\begin{split}
\mathbf{x}_{ij}
=h_{1\mathbf\Theta}\left([\mathbf{p}_j - \mathbf{p}_i;\mathbf{x}_j - \mathbf{x}_i]\right),\\
\mathbf{x}_{i} =h_{2\mathbf\Theta}\left([\mathbf{x}_{ij};\underset{j:(i, j) \in \mathcal{N}}{\operatorname{MAX}}{\mathbf{x}_{ij}}]\right);
\end{split}
\end{equation}
where $\mathbf{p}_i$ and $\mathbf{x}_i$ denote the coordinates and features of the $i$-th center point. The index $j$ defines the $j$-th neighbor of point $i$. The proposed graph convolution extracts features for each center point from the \textit{relative positions} and \textit{relative features} of its neighbors. The maxpooled features inside each neighborhood, ${\operatorname{MAX}}_{j:(i, j) \in \mathcal{N}}{\mathbf{x}_{ij}}$, enrich the tokens with global information from the local groups. 
Both $h_{1\mathbf\Theta}$ and $h_{2\mathbf\Theta}$ are two-layer MLPs with batch normalization and ReLU. 


\minorsection{Decoder $\mathbf{g}$: Feature Propagation with Global Representation Appending}
The goal of decoder $\mathbf{g}$ is to yield the desired output for each task.  For segmentation, we introduce Feature Propagation, a successful and widely used decoder design from PointNet++ \cite{qi2017pointnet++}, into the ST model. Feature Propagation gradually interpolates the feature map and concatenates it with point features from the tokenizer to produce individual representation for each point. Global representations, \ie the [CLS] token and the global maxpooled non-class tokens, are appended to each point. The output of the global representation appending for every point $\mathbf{x}_{i} $ in the segmentation task can be formalized as:
$
[\mathbf{x}_i;\operatorname{MAX}\left(\mathbf{x}\right);\operatorname{[CLS]}]
$.
In the case of classification, the global representation appending is formalized as: 
$
[\operatorname{MAX}\left(\mathbf{x}\right);\operatorname{[CLS]}]
$.
This \textit{global representation appending} technique enriches global information for both classification and segmentation and improves performance by non-trivial margins (see Sec. \ref{sec:ablation} for the ablation study).


\subsection{Pix4Point Pipeline}
\label{sec:pix4point_pipeline}
Another main argument of this work is that 3D point clouds are expensive to acquire, but images are easily available and could be exploited. To this end, we propose Pix4Point, a framework that enables improving PViT through image pretraining.
We illustrate the pipeline of Pix4Point in Fig. \ref{fig:pipeline}. It consists of three stages: (1) pretraining on images, (2) transferring image-pretrained weights to PViT, and (3) finetuning PViT on point cloud tasks. 

\minorsection{Pretraining Stage}
The goal of this stage is to utilize a large number of public images to pretrain the ST backbone of PViT. By default, we pretrain \textit{ViT-S} using the the self-supervised method MAE \cite{he2022mae} on \emph{ImageNet-1K} \cite{deng2009imagenet} dataset. Note that our Pix4Point is generally agnostic of the  pretraining strategy. Besides the aforementioned self-supervised pretraining, there are many other applicable strategies, \eg supervised training through DeiT \cite{touvron2021deit}. Refer to Sec. \ref{sec:ablation} for the effects of different pretraining strategies. 



\minorsection{Weight Transfer Stage}
The goal of this stage is to transfer the image-pretrained weights to the downstream point cloud network. 
Unlike previous methods that require 2D view projections or kernel inflation \cite{su15mvcnn, xu2021image2point}, this stage in Pix4Point is as simple as using the weights of the image-pretrained Transformer as an initialization for the backbone of our PViT network. This is possible because the exact same ST backbone (\eg ViT-S backbone) is used in both the image pretraining and the downstream point cloud tasks. 


\minorsection{Finetuning Stage}
The finetuning stage finetunes the image-pretrained ST backbone $\mathbf{F}$ for point cloud tasks. The tokenizer $\mathbf{t}$ and the task-specific decoder $\mathbf{g}$ of PViT are jointly trained from scratch during this fine-tuning stage. The loss for Pix4Point can be described as follows:
\begin{equation}
\begin{aligned} 
\argmin_{\boldsymbol{\theta}_{\mathbf{t}},\boldsymbol{\theta}_{\mathbf{F}}, \boldsymbol{\theta}_{\mathbf{g}}} &~~\sum_{i}^{B} L~\Big( \mathbf{g} \big(  \mathbf{F}\left( \mathbf{t}\left({\mathcal{X}}\right)\right)  \big)_i ~,~\mathbf{y}_i \Big), 
\label{eq:pipeline}
\end{aligned} 
\end{equation}
where $\{\mathbf{y}_i\}_{i=1}^B$ defines the labels of a mini-batch of input point clouds $\mathcal{X}$ and $L$ is a Cross-Entropy (CE) loss. 

\noindent\textbf{Why does Pix4Point Work?}
The 2D tokenizer and the 3D tokenizer project the input images and the point clouds into a shared token space $\mathcal{R}^C$, respectively, where each token from 2D or 3D is embedded as a vector of the same length $C$. 
Despite the domain shift between 2D and 3D and owing to the diverse large-scale image data in the pretraining stage, the ST backbone has learned to transform and mix the information of tokens in this shared token space. 
Therefore, it only takes a few finetuning epochs to tune ST and optimize the domain-specific tokenizer for the downstream point cloud tasks. Interestingly, we show (see Sec. \ref{sec:ablation}) that even when the image pretrained Transformer backbone is kept frozen, our proposed pipeline can still adequately recognize point clouds by training only the tokenizer and decoder in the downstream task.
This verifies our hypothesis that how to transform and mix information in the shared token space has been learned during image pretraining stage.

\minorsection{Comparison with Recent Methods}
The state-of-the-art methods for improved Standard Transformers on point clouds are Point-BERT \cite{yu2022pointbert} and Point-MAE \cite{pang2022pointmae}. Both methods find that the ST cannot achieve comparable results in point cloud tasks. They utilize self-supervised learning methods on point cloud data to improve performance.
In our work, we diverge from previous studies, and propose two contributions: (i) the PViT network that improves ST on point clouds through the P3E tokenizer and Feature Propagation decoder with global representation appending; (ii) the Pix4Point framework that exploits image pretraining for 3D point cloud understanding. 

==> figures/sectionsCVPR/relatedwork.tex <==
\section{Related Work}
\subsection{3D Point Cloud Understanding}
\minorsection{Point Cloud Networks} 
Due to breakthrough progress in deep learning technology \cite{krizhevsky2012alexnet,he2016resnet,qi2017pointnet,qi2017pointnet++}, current prevailing point cloud processing methods are entirely data-driven and consist of three main approaches: view-based \cite{su15mvcnn,hamdi2021mvtn,goyal2021simpleview}, voxel-based \cite{maturanaVoxNet3DConvolutional2015,graham2018sparseconv,choy2019minkowski}, and point-based~\cite{qi2017pointnet,qi2017pointnet++}. 
Among these three approaches, point-based methods, which directly take point clouds as input and process in their unstructured format, are receiving increasing attention, since there is no information loss. 
PointNet~\cite{qi2017pointnet}, the pioneering work of point-based methods, proposes to model the permutation invariance of points by restricting feature extraction to be pointwise. PointNet++~\cite{qi2017pointnet++} improves PointNet by further capturing local geometric structures. Most current point-based methods focus on the design of local modules \cite{wang2019dgcnn,li2018pointcnn,wu2019pointconv,thomas2019kpconv,li2019deepgcns,li2021deepgcn,qian2021pugcn,qian2021assanet,qian2022pointnext,zhao2021pointtransformer}. 
In this work, we pay attention to point-based methods, specifically, Transformer-based networks \cite{vaswani2017attention}, which have been proposed as a new paradigm for processing point clouds \cite{guo2021pct,zhao2021pointtransformer,yu2022pointbert}. 



\minorsection{2D to 3D Transfer Learning}
A straightforward means of transferring 2D learned representation to 3D is to use view-based methods. As a specific example, PointCLIP \cite{zhang2022pointclip} showed that a pretrained CLIP \cite{radfordLearningTransferableVisual2021} model can be used directly for zero-shot point cloud classification. More advanced methods leverage point-pixel correspondences \cite{liu20213d--2d,hamdi2021voint,wang2022p2p} between point clouds and multi-view images, where pointwise pseudo-labels can be generated from images to optimize a point cloud network. 
More recently, Image2Point \cite{xu2021image2point} presents a kernel inflation technique that expands 2D kernels of a 2D CNN into 3D kernels and further applies them to voxel-based point cloud understanding. 
However, these approaches lead to performance degradation. 
Multi-view methods can lead to non-ideal views, and a loss of geometric information \cite{strike,hamdi2021mvtn}, while kernel inflation only shows insignificant performance gains given the gap between 2D and 3D kernels \cite{xu2021image2point}. 
In this work, we present a novel pipeline that can directly utilize the Transformer pretrained on images for 3D point cloud tasks, without image projection or kernel inflation. 


\minorsection{Self-Supervised Learning on Point Clouds}
One prominent way to tackle the need for large labeled data is to rely on self-supervised learning (SSL) \cite{chen2020simple,caron2021dino}. Previous works in SSL for point clouds rely on pretext tasks \cite{Achlioptas2018generativepointcloud,sauder2019reconstruct} or auto-encoders \cite{Li2018SONetSN,Achlioptas2018generativepointcloud,wang2021occo,yan2022implicit}.
PointContrast \cite{Xie2020pointcontrast} proposes to generate two views of the point cloud with random transformations and ask the neural network to minimize the distance between matched points.
On the other hand, Point-BERT \cite{yu2022pointbert} and Point-MAE \cite{pang2022pointmae} propose masked auto-encoders to learn useful representations for 3D classification. 
Our method does not count on the availability of large amounts of point cloud data, as usually needed in SSL. Instead, we focus on how to utilize already available image data for pertaining point cloud networks.

\subsection{Transformers}
\minorsection{Specialized Transformer Architectures}
Based on its multi-head attention block, the Transformer \cite{vaswani2017attention} is believed to be the most successful architecture for natural language process (NLP). 
Vision Transformer (ViT) explores the direct application of this Transformer on image patches to solve vision tasks \cite{dosovitskiy2021vit}.
There is also an increasing interest in Transformer-like architectures for point cloud processing. 
Unfortunately, ST \cite{vaswani2017attention, dosovitskiy2021vit} cannot achieve results comparable to their convolutional counterparts in point cloud tasks \cite{yu2022pointbert}, mostly due to the small scale of point cloud data. This leads to a boom of specially designed variants of Transformer-based models \cite{yanPointasnlRobustPoint2020,hertzPointgmmNeuralGmm2020,guo2021pct,zhao2021pointtransformer,lai2022stratified}.
In contrast to these previous works that specialized the Transformer architecture, we maintain the same ST architecture and study means of improving its performance, by only changing its tokenizer and decoder. 


\minorsection{Transformer as a General Backbone}
\cite{lu_pretrained_2021} proposes a pretrained Transformer as a universal backbone for protein prediction and language understanding. 
Gato \cite{reed2022gato} is proposed to be a generalist agent that can perform tasks ranging from image captioning and language tasks to robot manipulation and reinforcement learning. 
Most recently, Omnivore \cite{Girdhar_2022_omnivore} proposes a vision Transformer model that works with multiple modalities such as videos and RGBD data, showing the benefit of 2D training in improving performance in different modalities. In our work, we utilize 2D image pretrained Transformers. Unlike Omnivore and Gato, our goal is to leverage these image-pretrained Transformers for point cloud tasks, which is under-studied. 


==> figures/tex/portionAblation.tex <==
\begin{figure}[t]
\centering
% \parbox[][5.2cm][c]{\linewidth}{
\centering
\includegraphics[width=1.0\linewidth]{src/datasetScale.pdf}
% }
% \subcaption{Effects of pretraining dataset scale}
% \vspace{-2em}
\caption{ \textbf{Effect of the Pretraining Dataset Size.} 
We show curves of downstream performance in S3DIS area 5 (val mIoU and mAcc) vs the portion of sampled ImageNet-1K used in pretraining. As observed, image-pretraining improves point cloud understanding, and the improvement is increased with the size of the pretraining dataset.
\todo{make this a table instead. }
}
\label{fig:dataset_scale}
\end{figure}

==> figures/tex/shapeNetCurve.tex <==
\begin{figure}[t]
\centering
\includegraphics[ width=0.98\linewidth]{src/shapeNet_train_curve.pdf}
\caption{ \textbf{Finetuning Epoch vs. Downstream Performance on Shape-Net Parts dataset.}The curves corresponds to
training from scratch are colored black, while the curves of Pix4point are colored in \R{red}. }
\label{fig:shapeNetCurve}
\end{figure}

==> sections/limitation.tex <==
\section{Limitation and Future Work}
While the scope of this work is to investigate the benefits of using image-based Transformers in the point cloud domain, a possible future work is to investigate \textit{cross-modality transfer learning or domain adaptation}. For example, it would be interesting to see whether language models can be used as an initialization for point clouds or image tasks and whether point clouds models can benefit language or image understanding?  Another promising future work is to jointly optimize both images and point clouds, creating \textit{a generalist vision Transformer} backbone that performs across the 2D and 3D domains. 



==> tables/Backbone.tex <==
%------------------------
% \begin{table*}[htb]
%  \small
% \centering
%   \caption{Backbone Setting.}
%     \label{tab:backbone}%
%     \begin{tabular}{ccccc|c|c|c}
%     \toprule
%   Dataset & Sample Ratio & Embedding Method &Group Size & Model & Validation ACC & No-pertrain OA & $\Delta$ \\
%     \hline
%  \rowcolor[rgb]{ 1,  1,  0} ScanObjectNN & 0.25  & KNN   & 32    & small & 0.840& 0.751& 0.09\\
%      ScanObjectNN & 0.5   & KNN   & 32    & small & 0.835 & {0.801} & {0.034} \\
%      ScanObjectNN & 0.25  & KNN   & 8     & small & {0.787} & {0.761} & {0.026} \\
%      ScanObjectNN & 0.25  & KNN   & 16    & small & {0.791} & {0.769} & {0.022} \\
%      ScanObjectNN & 0.25  & KNN   & 64    & small & {0.822} & {0.805} & {0.017} \\
%      ScanObjectNN & 0.25  & KNN   & 32    & tiny  & {0.812} & {0.758} & {0.054} \\
%      ScanObjectNN & 0.25  & KNN   & 32    & base  & {0.798} & {0.641} & {0.106} \\
%      ScanObjectNN & 0.25  & KNN   & 32    & large & {0.737} & {0.523} & {0.214} \\
%      ScanObjectNN & 0.25  & KNN   & 32    & huge  & {0.458} & {0.351} & {0.106} \\
%     ModelNet40 & 0.25  & KNN   & 32    & small & {0.939} & {0.937} & {0.002} \\
%      ScanObjectNN & 0.25  & Query-Ball & 32    & small & 0.831   & 0.732   & 0.099 \\
%      ScanObjectNN & 0.25  & Kmeans & 32    & small & 0.837   & 0.735   & 0.102 \\
%      ScanObjectNN & 0.25  & GCN   & 32    & small & 0.839   & 0.748   & 0.091 \\
% \bottomrule[1pt]
% \end{tabular}
% \end{table*}



\begin{table*}[!hp]
\tabcolsep=0.07cm
    \centering
\resizebox{0.98\linewidth}{!}{\begin{tabular}{ccccccc}
\toprule
 &   & Embedding,  &    &   \multicolumn{2}{c}{Classification Accuracy}& \\
\multicolumn{1}{c}{Dataset}&Sample Ratio &Group Size  & Model & With Pre-train & No pre-train& $\Delta$ \\ \midrule
ScanObjectNN & 0.0625  & KNN, 32 & small & 82.44&78.63&3.81\\
 & 0.125  & KNN, 32    & small         & 83.1& 80.81&2.29\\
  & 0.25  & KNN, 32    & small       &  84     & 80.99&3.01\\
      & 0.5   & KNN,32    & small   & 82.51   & 81.26& 1.25\\
       & 0.25  & KNN,8     & small & 80.99    & 79.8& 1.19 \\
       & 0.25  & KNN,16    & small &  83.03    & 81.8 & 1.23 \\
       & 0.25  & KNN,64    & small & 82.1        &81    & 1.1 \\
       & 0.25  & KNN,32    & tiny  &81.92      & 79.56 &2.36 \\
       & 0.25  & KNN,32    & base  &79.84    & 64.64 & 15.2 \\
       & 0.25  & KNN,32    & large & 74.53    &52.74 & 21.79 \\
       & 0.25  & KNN,32    & huge  & 46.04    & 35.93 & 10.11 \\
       & 0.25  & Query-Ball,32    & small & 82.4  &80.52  & 1.88\\
\midrule
 ModelNet40 & 0.25  & KNN,32    & small & {0.939} & {0.937} & {0.002} \\
\bottomrule
\end{tabular}
}
\vspace{2pt}
    \caption{\textbf{Ablation on Backbone Setting}.}
     \label{tab:backbone}
\end{table*}

==> tables/WithSota.tex <==
\begin{table}[H]
  \centering%\multicolumn{3}{ r}
  \caption{3D Point Cloud Classification on ScanObjectNN and ModelNet40}
      \label{tab:sota}
\begin{tabular}{|c|c|c|}
    Approach& OA(ScanObjectNN)  &OA (ModelNet) \\
    \hline
  PointMLP~\cite{maRethinkingNetworkDesign2022}  &85.7& 94.5\\
    \hline
 Point-MAE~\cite{pangMaskedAutoencodersPoint2022} & 85.2& 94.0\\
  \hline
APP-Net~\cite{luAPPNetAuxiliarypointbasedPush2022}& 84.1&93.6\\
 \hline
Ours& 84.0& 92.1 \\ 
 \hline
Point-BERT~\cite{yu2021point}& 83.1&93.8 \\
 \hline
 MVTN~\cite{hamdi2021mvtn} & 82.8& 93.8
\end{tabular}
\end{table}

==> tables/architectureAblation.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[tb]
  \centering
  \caption{ \textbf{Ablation Study: Choices of the Global Representation on 3D Segmentation of S3DIS Srea 5}.}
    \begin{tabular}{l|c|c}
    \toprule
    Method
    % &	OA
    &	mAcc&	mIoU\\
\midrule
    NONE
    &  73.0$\pm$0.3  &  66.8$\pm$0.5  \\
    CLS  
    & \textbf{74.0}$\pm$0.9&	67.3$\pm$0.6\\
    CLS;MAX \textbf{(ours)}
    &  73.7$\pm$0.6  &  \textbf{67.5}$\pm$0.9  \\
    CLS;MAX;AVG
    % &  89.3$\pm$0.2  
    &  73.6$\pm$0.5  &  66.9$\pm$0.1  \\
    \bottomrule
    \end{tabular}%
  \label{tab:ablate_globals}%
\end{table}%



==> tables/frozen.tex <==
\begin{table}[h]
\centering
\caption{\textbf{Semantic segmentation results on S3DIS area 5 of Pix4Point with \textit{frozen} Transformer backbones.}
}
\label{tab:s3dis_frozen}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{ l | l l l}
\toprule[1pt]
Method
 &   mAcc  &  mIoU \\
\toprule
random initialized& $51.8\pm0.5$ &	$44.3\pm0.2$ \\
\midrule
ShapNetPart sup. training & \todo{exp}\\
Point-MAE ShapeNet pretraining & \reshll{$53.9\pm1.6$}{+}{2.1}	& \reshll{$46.5\pm1.8$}{+}{2.2}\\ 
\midrule
DeiT ImageNet pretraining & 
\reshll{$58.5\pm1.0$}{+}{6.7} &	\reshll{$51.4\pm1.2$}{+}{7.1}\\
DINO ImageNet pretraining &\reshll{$58.8\pm0.2$}{+}{7.0} &	\reshll{$52.0\pm0.0$}{+}{7.7} \\
\bottomrule[1pt]
\end{tabular}}
\end{table}

==> tables/modelnet.tex <==
% % ModelNet Classification 
\begin{table}[ht]
\centering
\caption{\textbf{Shape Classification on ModelNet40.} Image pretraining improves classification performance on ModelNet40.}
\label{tab:modelnet40}
\resizebox{\linewidth}{!}{
\begin{tabular}{ l | l l ll }
\toprule
Method  & mAcc & OA  & Params. & FLOPs \\
% & Params. & FLOPs & Throughput \\
\midrule
% 		3DShapeNets~\shortcite{wu2015modelnet}  & 77.3 & 84.7 \\
% 		VoxNet~\shortcite{maturana2015voxnet}  & 83.0 & 85.9 \\
% 		Subvolume~\shortcite{qi2016volumetric}  & 86.0 & 89.2 \\
% 		MVCNN~\shortcite{su15mvcnn}  & -- & 90.1 \\
% 		A-SCN~\shortcite{xie2018attentional}  & 87.6 & 90.0 \\
% 		Set Transformer~\shortcite{lee2019set}  & -- & 90.4 \\
% 		PAT~\shortcite{yang2019modeling}  & -- & 91.7 \\
% 		SpecGCN~\shortcite{wang2018local}  & -- & 92.1 \\
PointNet~\shortcite{qi2017pointnet} & 86.2 & 89.2& 3.5 & 0.9\\
% & 3.5 & 0.9 & 4212\\ % checked from PointNet
PointNet++~\shortcite{qi2017pointnet++} & - & 91.9& 1.5  & 1.7 \\
% & 1.5  & 1.7 & 1872 \\ % checked from pointConv
PointCNN~\shortcite{li2018pointcnn} & 88.1 & 92.2& 0.6 & -  \\
% & 0.6 & - & 44 \\ % checked from PointCNN
% 		PointWeb~\shortcite{zhao2019pointweb}  & 89.4 & 92.3 \\
% 		SpiderCNN~\shortcite{xu2018spidercnn}  & -- & 92.4 \\
PointConv~\shortcite{wu2019pointconv} & -- & 92.5 
& - & -\\ % checked from pointConv
% 		Point2Sequence~\shortcite{liu2019point2sequence}  & 90.4 & 92.6 \\
% 		ShellNet~\shortcite{zhang2019shellnet} & - & 92.8 \\
KPConv~\shortcite{thomas2019kpconv} & - & 92.9
& - & -\\ % checked from KPConv
DGCNN~\shortcite{wang2019dgcnn} & 90.2 & 92.9
& 1.8 & 4.8 \\ % & 90.7 & 93.5 is 2048 points results 
DeepGCN \shortcite{li2021deepgcn}   & 90.9  & 93.6
& 2.2 & 3.9\\ % the best from https://github.com/lightaime/deep_gcns_torch/blob/master/examples/modelnet_cls/README.md is  & 90.9  & 93.6
ASSANet-L ~\shortcite{qian2021assanet} & - & 92.9
&- & - \\ % checked from ASSA-Net
Point Cloud Transformer~\shortcite{guo2021pct} & - & 93.2
&- & - \\
% & 	2.88	\\ % checked from PCT
Point Transformer~\shortcite{zhao2021pointtransformer} & 90.6 & 93.7 
&- & - \\ % checked 
% 		InterpCNN~\shortcite{mao2019interpolated}  & -- & 93.0 \\
% 		Grid-GCN~\shortcite{xu2020grid} & 91.3 & 93.1\\
% 		PosPool~\shortcite{liu2020closer} & - & 93.2 \\
CurveNet~\shortcite{xiang2021walk}  & - & 94.2&- & -   \\ % checked from CurveNet, also 1024 points,  94.2 with voting
PointMLP~\shortcite{ma2022pointmlp} & 91.4 & 94.5
& 13.2 & 31.3 \\ % ma: 91.4, oa: 94.5
\midrule
% PatchFormer~\shortcite{cheng2022patchformer}  & - & - &  - & - \\ 
%Fast PointTransformer~shortcite{park2022fpt} & - & - &  - & - \\
Point-BERT~\shortcite{yu2022pointbert} &  - & 	93.8&-& -	\\ 
% &  - & -& - \\
Point-MAE~\shortcite{pang2022pointmae} &  -&	94.0
&253.0 & -\\
% \midrule  
\gr Pix4Point (scratch)  &$90.0\pm0.9$  &$93.7\pm0.5$ 
&23.1 & -\\
\gr \textbf{Pix4Point (pretrained)}& \reshll{$90.1\pm0.2$}{+}{0.1}
&\reshll{$93.9\pm0.1$} {+}{0.2} 
&23.1 & -\\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/scanobjectnn_modelnet.tex <==
% \begin{wraptable}{r}{0.7\textwidth}
\begin{table*}[tb]
\small
\centering
\caption{\textbf{3D Object classification on real-scanned dataset ScanObjectNN and CAD model dataset ModelNet40.
\todo{@Gordon, performance on ModelNet40 must be increased.}
} 
}
\label{tab:cls_scanobjectNN}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{l|ll|ll}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{ScanObjectNN}}  & \multicolumn{2}{c}{\textbf{ModelNet40}} \\
& OA & mAcc & OA & mAcc \\ % & FLOPs Params.  & Throughput
\midrule
PointNet~\cite{qi2017pointnet}&68.2  &63.4 & 89.2  & 86.2 \\ % flops=& 0.94
PointNet++~\cite{qi2017pointnet++} & 77.9 &75.4 & 91.9   & - \\ % flops=& 1.7
% SpiderCNN~\cite{xu2018spidercnn} &69.8 &73.7 \\
PointCNN~\cite{li2018pointcnn}&78.5  &75.1 & 92.2  & 88.1 \\
DGCNN~\cite{wang2019dgcnn} &78.1 &73.6 & 92.9   & 90.2  \\  % flops=& 4.82
% BGA-DGCNN~\cite{uy2019revisiting} &75.7 &79.7 \\
% BGA-PN++~\cite{uy2019revisiting} &77.5 &80.2 \\
% DRNet~\cite{qiu2021dense}  &80.3  &78.0 & - & -\\
% SimpleView~\cite{goyal2021simpleview} & - &80.5 &0.8 \\
% GBNet~\cite{qiu2022gbnet} & 80.5 & 77.8 & - & -\\
% PRANet~\cite{cheng2021net}&82.1  & 79.1&  - & - \\ % flops=& 348
% DeepGCN \cite{li2021deepgcn}  & -&- &  93.6&90.9 \\ % the best from https://github.com/lightaime/deep_gcns_torch/blob/master/examples/modelnet_cls/README.md is  & 90.9  & 93.6
% ASSANet-L ~\cite{qian2021assanet} & -&- &92.9&-  \\ % checked from ASSA-Net
% CurveNet~\cite{xiang2021walk}   & -&- &93.8  &- \\ % checked from CurveNet, also 1024 points,  94.2 with voting

% MVTN~\cite{hamdi2021mvtn} & 82.8 & -& - & - \\
PointMLP~\cite{ma2022pointmlp}  & $85.4\pm1.3$ & $83.9\pm1.5$ & 93.7$\pm$0.2& 90.9$\pm$0.4 \\ % flops=& 31.4
% DeltaNet~\cite{Wiersma2022DeltaConv} & 84.7 &  \\
% RepSurf-U~\cite{ran2022surface} & \textbf{86.0} & 83.1 & 6.8 & - \\  
\midrule
% PCTransformer~\cite{guo2021pct} & - &- & - & -\\ % from PCT verified at area 5
% Point Transformer~\cite{zhao2021pointtransformer} & - &- & - & - \\ % from pointTransofrmer verified at area5 
% PatchFormer~\cite{cheng2022patchformer}  & - & - &  - & - \\ 
% Fast PointTransformer~cite{park2022fpt} & - & - &  - & - \\
% \midrule
Point-BERT~\cite{yu2022pointbert} & 83.1 & - &  93.8 & - \\
Point-MAE~\cite{pang2022pointmae} & 85.2 & - &  94.0 & - \\
\gr Pix4Point (scratch) &{$85.5\pm0.6$} &	$83.8\pm0.2$  & $92.0\pm0.5$ &$88.3\pm0.9$ \\ % 
\gr \textbf{Pix4Point (pretrained)} &  \reshll {$\textbf{86.4}\pm0.2$}{+}{0.9} &   \reshll {$\textbf{84.6}\pm0.6$}{+}{0.8}& \reshll{$92.5\pm0.1$} {+}{0.5}& \reshll{$89.2\pm0.2$}{+}{0.9} \\ % flops=& 1.6
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/tokenizer.tex <==
\begin{table}[tb]
\centering
\caption{\textbf{Ablate the Network Design of PViT on S3DIS Area 5.}
All backbones are initialized with the same Pix4Point image pretraining. PViT+Pix4Point is used as the baseline.
The proposed progressive tokenizer with graph convolutions using relative features (P3E) and the global representation appending contribute to significant performance improvements (over $2$ mIoU).   
}
\label{tab:ablate_tokenizer}
\vspace{-0.5em}
\begin{tabular}{l|c|c}
\toprule
\textbf{Conponent ablated}&\textbf{mIoU}&\textbf{mAcc}\\
\midrule
baseline (PViT+Pix4Point) & 69.6 & 75.2 \\
\bluerow Progressive tokenizer & 65.3 & 71.4 \\
\bluerow Relative feature input & 61.6 & 67.6 \\
\greenrow Global representation (only max) & 68.5 & 74.0 \\
\greenrow  Global representation (only [CLS]) & 68.2 & 73.8	\\
\greenrow  Global representation (none) & 67.5 & 73.2	\\
% $[\mathbf{p}_j - \mathbf{p}_i;\mathbf{x}_j]$ 
% &   $56.4\pm0.9$  
% &  $62.8\pm0.7$  \\
% $[\mathbf{p}_j;\mathbf{x}_j - \mathbf{x}_i]$  
% &$62.3\pm0.2$ 
% & $68.8\pm0.2$\\
% $[\mathbf{p}_j;\mathbf{x}_j]$ 
% &  $56.6\pm0.3$  
% &  $63.3\pm0.4$  \\
% $[\mathbf{p}_j - \mathbf{p}_i;\mathbf{x}_j - \mathbf{x}_i]$ \textbf{(Ours)}
% &   $\textbf{65.6}\pm0.5$ 
% &   $\textbf{71.8}\pm0.5$\\ 
\bottomrule
\end{tabular}%
\vspace{-4mm}
\end{table}%

